ARGUS: Seeing the Influence of Narrative Features on Persuasion in Argumentative Texts

Can narratives make arguments more persuasive? And to this end, which narrative features matter most? Although stories are often seen as powerful tools for persuasion, their specific role in online, unstructured argumentation remains underexplored. To address this gap, we present ARGUS, a framework for studying the impact of narration on persuasion in argumentative discourse. ARGUS introduces a new ChangeMyView corpus annotated for story presence and six key narrative features, integrating insights from two established theoretical frameworks that capture both textual narrative features and their effects on recipients. Leveraging both encoder-based classifiers and zero-shot large language models (LLMs), ARGUS identifies stories and narrative features and applies them at scale to examine how different narrative dimensions influence persuasion success in online argumentation.

==> ACM2026/sections/analysis_old.tex <==
\section{Narrativity and Persuasion}
\label{analysis}
\textit{Does narrative predict persuasion outcomes on ChangeMyView}? To test our main research question, we use the corpus of \citet{tan+etal:16a} (Section~\ref{sec:data}), taking \emph{Deltas} as proxies of persuasiveness. We exclude discussions and comments posted by moderators or system accounts as well as comments authored by users labeled as `[deleted]' in the corpus, obtaining 963,253 comments. 
On these, we apply our best-performing narrativity and narrative features models, For \textit{Story}, we use the scalar model given its higher performance, identifying 158,641 (16\%) story comments.

The study is carried out in three steps:
\begin{enumerate}
    \item We test whether narrativity predicts persuasion.
    \item We examine which narrative features drive this effect.
    \item We assess whether structural and perceptual dimensions interact in persuasion. 
\end{enumerate}
 
All analyses use mixed-effects logistic regression to estimate the probability that a comment receives a \emph{Delta}, including random intercepts for comment authors and original posters to account for repeated participation, and controlling for comment length. All continuous predictors are z-standardized.

\subsection{Are narrative arguments more likely to persuade?} First we test if narrativity predicts persuasion success by modeling delta by narrativity score and comment length, and narrative presence and comment length:
\begin{itemize}
    \item \(Model_{1}\): \(Delta \sim  Story_{scalar} + Text_{length} + (1|Author) + (1|OPAuthor)\) 
    \item \(Model_{2}\): \(Delta \sim  Story_{binary} + Text_{length} + (1|Author) + (1|OPAuthor)\)
\end{itemize}

Results, in Table~\ref{tab:analysis_m1_m2}, show that narrativity has a strong positive effect on \emph{Delta} ($\beta = 0.45$, $p < 0.001$): a one unit increase in narrativity raises persuasion odds by about 57\% (OR $\approx 1.57$). A model using the binary story label as predictor yields a comparable effect ($\beta = 0.62$, $p < 0.001$, OR $\approx 1.86$). Comment length also increases persuasion likelihood of \emph{Delta} ($\beta = 0.36$–$0.42$, OR $\approx 1.43$–$1.52$), but narrativity provides a robust persuasive advantage beyond comment length and differences between authors, which are controlled for in the model.

\begin{table}[h]
\caption{Results of \(Model_{1}\) and \(Model_{2}\). $\boldsymbol{\beta}$= log-odds coefficients, \textbf{SE} = standard error, \textbf{z} = the Wald test statistic, $\boldsymbol{p}$= p-value, and \textbf{OR} = odds ratio (computed as $\exp(\boldsymbol{\beta})$).}
\label{tab:analysis_m1_m2}
\centering
\begin{tabular}{l|ccccc}
\toprule
\textbf{Predictor} & $\boldsymbol{\beta}$ & \textbf{SE}  & \textbf{z} & $\boldsymbol{p}$ & \textbf{OR} \\ 
\midrule
\multicolumn{6}{c}{\textbf{\(Story_{scalar} Predictor\) }}\\
\midrule
Intercept & -5.65 & 0.03 & 39.26 & $< 0.001$ &  - \\
Story\(_{scalar}\) & 0.45 & 0.01 & 39.26 & $< 0.001$ &  1.57 \\
Text\(_{length}\)    & 0.36 &  0.01 & 53.88 & $< 0.001$ & 1.52 \\
\midrule
\multicolumn{6}{c}{\textbf{\(Story_{binary} Predictor\) }}\\
\midrule
Intercept & -5.69 & 0.03 & -170.84 & $< 0.001$ &  - \\
Story\(_{binary}\) & 0.62 & 0.03 & 25.18 & $< 0.001$ & 1.86 \\
Text\(_{length}\)    & 0.42 & 0.01 & 67.31 & $< 0.001$ & 1.43\\
\bottomrule
\end{tabular}
\end{table}


\subsection{Which specific narrative features make a story persuasive?} 

Before testing what story features contribute to persuasion, we first verify that they reliably predict narrativity. We create two composite measures: \textit{structural score}, defined as the average of \textit{Agency} and \textit{Event Sequencing}, and \textit{response score}, defined as the average of \textit{Suspense}, \textit{Curiosity}, and \textit{Surprise}. Using these predictors and controlling for the comment length, we estimate two models: one predicting a story presence and one predicting a continuous narrativity score:

\begin{itemize}
    \item \(Model_{3}\): \(Story_{scalar} \sim Structural_{score} + Response_{score} + Text_{length}\)
    \item \(Model_{4}\): \(Story_{binary} \sim Structural_{score} + Response_{score} + Text_{length}\)
\end{itemize}

Results are reported in Table~\ref{tab:analysis_m3_m4}. Both structural and response scores are strong positive predictors of narrativity. In the logistic model predicting the binary story label, increases in both composite scores substantially raise the likelihood that a text is classified as a story, while text length is negatively associated with story classification. In the linear model predicting continuous story score, structural and response scores again show large positive effects, confirming that the composite narrative features capture the core dimensions of narrativity. 

\begin{table}[h]
\caption{Results of \(Model_{3}\) and \(Model_{4}\). $\boldsymbol{\beta}$= log-odds coefficients, \textbf{SE} = standard error, \textbf{z} = the Wald test statistic, \textbf{t} = the t-test statistic, $\boldsymbol{p}$= p-value, \textbf{OR} = odds ratio (computed as $\exp(\boldsymbol{\beta})$), and $\boldsymbol{\eta^2}$ = partial eta squared. \(Model_{3}\) adjusted $\boldsymbol{R^2}$= 0.77.}
\label{tab:analysis_m3_m4}
\centering
\begin{tabular}{l|ccccc}
\toprule
% \textbf{Predictor} & $\boldsymbol{\beta}$ & \textbf{SE}  & \textbf{z/t} & $\boldsymbol{p}$ & \textbf{OR} \\ 
% \midrule
\multicolumn{6}{c}{\textbf{ \(Story_{scalar} \) }}\\
\midrule
\textbf{Predictor} & $\boldsymbol{\beta}$ & \textbf{SE}  & \textbf{t} & $\boldsymbol{p}$ & $\boldsymbol{\eta^2}$ \\ 
\midrule
Intercept & 0.00 & 0.00 & 0.00 &1.00  &  - \\
Response\(_{score}\) & 0.49 &0.00 &715.34 & $< 0.001$ & 0.35  \\
Structural\(_{score}\) & 0.53 & 0.00&766.55&$< 0.001$ &  0.38 \\
Text\(_{length}\)    & -0.06 &  0.00 &-80.05&$< 0.001$  & 0.01\\
\hline
\multicolumn{6}{c}{\textbf{\(Story_{binary} \)}}\\
\midrule
\textbf{Predictor} & $\boldsymbol{\beta}$ & \textbf{SE}  & \textbf{z} & $\boldsymbol{p}$ & \textbf{OR} \\ 
\hline
Intercept & -2.76 & 0.01 & -393.28 & $< 0.001$ & -  \\
Response\(_{score}\) & 1.17 & 0.01 & 130.49 & $< 0.001$ & 3.22 \\
Structural\(_{score}\) & 1.91 &  0.01& 275.40 & $< 0.001$& 6.75 \\
Text\(_{length}\)    & -0.39 & 0.00 & -84.55 & $< 0.001$ & 0.68\\
\bottomrule
\end{tabular}
\end{table}

Having established this, we next examine how these composite scores contribute to persuasive outcomes, focusing only on comments predicted to contain a story (16.5\%, 158,641 comments), using the following model:

\begin{itemize}
    \item \(Model_{5}\): \(Delta \sim Structural_{score} + Response_{score} + Text_{length} + (1|Author) + (1|OPAuthor)\)
\end{itemize}


Results are reported in Table~\ref{tab:analysis_m5}. Both narrative feature composites are positively associated with persuasion. Response score has a small but significant positive effect ($\beta = 0.07$, $p = 0.014$), while structural score shows a larger and more robust effect ($\beta = 0.10$, $p < 0.001$). Text length remains a strong predictor of persuasion ($\beta = 0.39$, $p < 0.001$). In terms of effect sizes, a one-unit increase in response score increases the odds of persuasion by about 7\% (OR $\approx 1.07$), while a one-unit increase in structural score increases the odds by about 11\% (OR $\approx 1.11$). 

\begin{table}[h]
\caption{Results of \(Model_{5}\). $\boldsymbol{\beta}$= log-odds coefficients, \textbf{SE} = standard error, \textbf{z} = the Wald test statistic, $\boldsymbol{p}$= p-value, and \textbf{OR} = odds ratio (computed as $\exp(\boldsymbol{\beta})$).}
\label{tab:analysis_m5}
\centering
\begin{tabular}{l|ccccc}
\toprule
\textbf{Predictor} & $\boldsymbol{\beta}$ & \textbf{SE}  & \textbf{z} & $\boldsymbol{p}$ & \textbf{OR} \\ 
\midrule
Intercept & -4.74 & 0.06 & -85.97 & $< 0.001$ &  - \\
Response\(_{score}\) & 0.07 & 0.03 & 2.46 & $0.014$ & 1.07 \\
Structural\(_{score}\) & 0.10 & 0.02 & 4.19 & $< 0.001$& 1.11\\
Text\(_{length}\) & 0.39 & 0.01 & 26.61 & $< 0.001$ & 1.48 \\
\bottomrule
\end{tabular}
\end{table}


% TEMP

\begin{table}[h]
\caption{Results of \(Model_{5}\). \textbf{FULLDATASET }$\boldsymbol{\beta}$= log-odds coefficients, \textbf{SE} = standard error, \textbf{z} = the Wald test statistic, $\boldsymbol{p}$= p-value, and \textbf{OR} = odds ratio (computed as $\exp(\boldsymbol{\beta})$).}
\label{tab:analysis_m5_temp}
\centering
\begin{tabular}{l|ccccc}
\toprule
\textbf{Predictor} & $\boldsymbol{\beta}$ & \textbf{SE}  & \textbf{z} & $\boldsymbol{p}$ & \textbf{OR} \\ 
\midrule
Intercept & -5.70 & 0.03 & -175.32 & $< 0.001$ &  - \\
Response\(_{score}\) & 0.59 & 0.02 & 30.24 & $< 0.001$ & 1.80 \\
Structural\(_{score}\) & 0.09 & 0.01 & 7.80 & $< 0.001$ & 1.09\\
Text\(_{length}\) & 0.30 & 0.01 & 39.91 & $< 0.001$ &  1.35\\
\bottomrule
\end{tabular}
\end{table}

We then examine the effects of individual narrative elements on persuasion by predicting \emph{Delta} using models that include each fine-grained feature separately:

\begin{itemize}
    \item \(Model_{6}\): \(Delta \sim Agency_{scalar} + Event Sequencing_{scalar} + Surprise_{scalar} + Suspense_{scalar} + Curiosity_{scalar} + Text_{length} + (1|Author) + (1|OPAuthor)\)
 \item \(Model_{7}\): \(Delta \sim Agency_{binary} + Event Sequencing_{binary} + Surprise_{binary} + Suspense_{binary} + Curiosity_{binary} + Text_{length} + (1|Author) + (1|OPAuthor)\)
\end{itemize}



Results are reported in Table~\ref{tab:analysis_m6_m7}. When entered as scalar predictors, \textit{Event Sequencing} ($\beta = 0.12$, $p < 0.001$) and \textit{Curiosity} ($\beta = 0.15$, $p < 0.001$) show positive associations with persuasion. \textit{Surprise} exhibits a significant negative effect ($\beta = -0.11$, $p = 0.006$), while \textit{Agency} and \textit{Suspense} do not show significant effects.

When narrative elements are instead modeled as binary indicators, the pattern changes. In this case, the presence of \textit{Surprise} shows a large positive association with persuasion, while the effects of \textit{Event Sequencing}, \textit{Suspense}, and \textit{Curiosity} are more modest. \textit{Agency} again does not reach statistical significance.

\begin{table}[h]
\caption{Results of \(Model_{6}\) and \(Model_{7}\).  $\boldsymbol{\beta}$= log-odds coefficients, \textbf{SE} = standard error, \textbf{z} = the Wald test statistic, $\boldsymbol{p}$= p-value, and \textbf{OR} = odds ratio (computed as $\exp(\boldsymbol{\beta})$).}
\label{tab:analysis_m6_m7}
\centering
\begin{tabular}{l|ccccc}
\toprule
\textbf{Predictor} & $\boldsymbol{\beta}$ & \textbf{SE}  & \textbf{z} & $\boldsymbol{p}$ & \textbf{OR} \\ 
\midrule
\multicolumn{6}{c}{Scalar Predictors}\\
\midrule
Intercept & -4.74 & 0.06 & -86.20 & $< 0.001$ &  -\\
Agency\(_{scalar}\)      & -0.01 & 0.03  & -0.30 & 0.766 & 0.99 \\
Event Sequencing\(_{scalar}\)      & 0.12 & 0.03  & 3.78 & $< 0.001$ & 1.13  \\
Suspense\(_{scalar}\)      & 0.03 & 0.03  &0.78& 0.438 &1.03\\
Curiosity\(_{scalar}\)      & 0.15 & 0.04 & 3.78 & $< 0.001$ & 1.16 \\
Surprise\(_{scalar}\)      & -0.11 & 0.04 & -2.73 & $0.006$ & 0.89  \\
Text\(_{length}\)    &  0.38 & 0.02 & 24.15 & $< 0.001$ & 1.46 \\
\midrule
\multicolumn{6}{c}{Binary Predictors}\\
\midrule
Intercept & -6.48 & 0.39 & -16.66 & $< 0.001$ & -\\
Agency\(_{binary}\)      & 0.06 &0.04& 1.33 & 0.18 &1.06\\
Event Sequencing\(_{binary}\)      & 0.09 & 0.04  & 2.04& 0.04 & 1.09 \\
Suspense\(_{binary}\)      &0.13& 0.06  & 2.18 & 0.03 &  1.14 \\
Curiosity\(_{binary}\)      & 0.92 & 0.40 & 2.30 & 0.02 &2.51\\
Surprise\(_{binary}\)      & 0.69 &  0.16 &4.33& $< 0.001$ &2.00\\
Text\(_{length}\)    & 0.39 &0.01& 27.45 & $< 0.001$ & 1.48  \\
\bottomrule
\end{tabular}
\end{table}

% TEMP
\begin{table}[h]
\caption{Results of \(Model_{6}\) and \(Model_{7}\). \textbf{FULLDATASET }$\boldsymbol{\beta}$= log-odds coefficients, \textbf{SE} = standard error, \textbf{z} = the Wald test statistic, $\boldsymbol{p}$= p-value, and \textbf{OR} = odds ratio (computed as $\exp(\boldsymbol{\beta})$).}
\label{tab:analysis_m6_m7_temp}
\centering
\begin{tabular}{l|ccccc}
\toprule
\textbf{Predictor} & $\boldsymbol{\beta}$ & \textbf{SE}  & \textbf{z} & $\boldsymbol{p}$ & \textbf{OR} \\ 
\midrule
\multicolumn{6}{c}{Scalar Predictors}\\
\midrule
Intercept & -5.72 & 0.03 & -175.572 & $< 0.001$ &  -\\
Agency\(_{scalar}\)      & 0.03 & 0.01  & 2.453 & 0.01 & 1.03 \\
Event Sequencing\(_{scalar}\)      & 0.06 & 0.02  & 3.59 & $< 0.001$ & 1.06 \\
Suspense\(_{scalar}\)      & 0.15 & 0.03  &4.90&$< 0.001$ & 1.16\\
Curiosity\(_{scalar}\)      & 0.60 & 0.04 & 15.865 & $< 0.001$ & 1.82 \\
Surprise\(_{scalar}\)      & -0.11 & 0.04 & -2.83 & $0.005$ &  0.89 \\
Text\(_{length}\)    &  0.30 & 0.01 & 37.56 & $< 0.001$ & 1.35 \\
\midrule
\multicolumn{6}{c}{Binary Predictors}\\
\midrule
Intercept & -6.43 & 0.04 & -151.452 & $< 0.001$ & -\\
Agency\(_{binary}\)  & 0.16 & 0.04 & 4.37 & $< 0.001$ & 1.17 \\
Event Sequencing\(_{binary}\)      & 0.17 & 0.03  & 5.07 & $< 0.001$ & 1.19 \\
Suspense\(_{binary}\)      & 0.30 & 0.03  & 9.85 & $< 0.001$ & 1.35  \\
Curiosity\(_{binary}\)      & 0.72 & 0.04 & 16.28 & $< 0.001$ & 2.05 \\
Surprise\(_{binary}\)      & 0.41 &  0.04 &10.55& $< 0.001$ & 1.51 \\
Text\(_{length}\)    & 0.33 & 0.01 & 45.49 & $< 0.001$ & 1.39  \\
\bottomrule
\end{tabular}
\end{table}






\subsection{Do text- and reader-oriented features reinforce each other in persuasion?}

Finally, we test whether text- and reader-oriented features interact in shaping persuasion. We use the two composite measures: \textit{structural score} and \textit{response score}, and use their interaction to predict delta:
\begin{itemize}
    \item \(Model_{8}\): \(Delta \sim Structural_{score} * Response_{score} + Text_{length} + (1|Author) + (1|OPAuthor)\)
\end{itemize}

Results, in Table~\ref{tab:analysis_m8}, show a significant negative interaction between structural and response features ($\beta = -0.11$, $p < 0.001$). While structural features are positively associated with persuasion ($\beta = 0.13$, $p < 0.001$), the main effect of response features is not statistically significant once the interaction is included ($\beta = 0.05$, $p = 0.109$).


\begin{table}[h]
\caption{Results of \(Model_{8}\). $\boldsymbol{\beta}$= log-odds coefficients, \textbf{SE} = standard error, \textbf{z} = the Wald test statistic, $\boldsymbol{p}$= p-value, and \textbf{OR} = odds ratio (computed as $\exp(\boldsymbol{\beta})$).}
\label{tab:analysis_m8}
\centering
\begin{tabular}{l|ccccc}
\toprule
\textbf{Predictor} & $\boldsymbol{\beta}$ & \textbf{SE}  & \textbf{z} & $\boldsymbol{p}$ & \textbf{OR} \\ 
\midrule
Intercept & -4.68 & 0.06 & -84.14 & $< 0.001$  & - \\
Structural\(_{score}\)      & 0.13 &  0.02 & 5.74& $< 0.001$ & 1.14  \\
Response\(_{score}\)      & 0.05 & 0.03 & 1.60 & 0.109 &  1.05\\
Structural\(_{score}\):Response\(_{score}\)     & -0.11 & 0.02 & -5.69 & $< 0.001$ & 0.90\\
Text\(_{length}\)    &  0.39 & 0.01 & 26.60 & $< 0.001$& 1.48 \\
\bottomrule
\end{tabular}
\end{table}

% TEMP
\begin{table}[h]
\caption{Results of \(Model_{8}\). \textbf{FULLDATASET} $\boldsymbol{\beta}$= log-odds coefficients, \textbf{SE} = standard error, \textbf{z} = the Wald test statistic, $\boldsymbol{p}$= p-value, and \textbf{OR} = odds ratio (computed as $\exp(\boldsymbol{\beta})$).}
\label{tab:analysis_m8_temp}
\centering
\begin{tabular}{l|ccccc}
\toprule
\textbf{Predictor} & $\boldsymbol{\beta}$ & \textbf{SE}  & \textbf{z} & $\boldsymbol{p}$ & \textbf{OR} \\ 
\midrule
Intercept & -5.54 & 0.03 & -165.88 & $< 0.001$  & - \\
Structural\(_{score}\)      & 0.48 &  0.03 & 18.29& $< 0.001$ &  1.62 \\
Response\(_{score}\)      & 0.46 & 0.02 & 21.60 & $< 0.001$  &  1.58\\
Structural\(_{score}\):Response\(_{score}\)     & -0.28 & 0.02 & -15.92 & $< 0.001$ & 0.76\\
Text\(_{length}\)    &  0.30 & 0.01 & 41.18 & $< 0.001$&  1.35\\
\bottomrule
\end{tabular}
\end{table}

\subsection{Discussion}

Across all analyses, narrativity is consistently associated with persuasion on \textit{ChangeMyView}. Comments that are higher with narrative are more likely to receive a \emph{Delta}, even after controlling for comment length and differences between authors and original posters. This pattern holds whether narrativity is measured as a continuous score or as a binary label, showing that both the presence of a story and the degree of narrativity contribute to persuasive success. This finding differs from prior conclusions by \citet{antoniak-etal-2024-people} and \citet{nabhani-etal-2025-storytelling}, who find weaker or more limited effects of narrativity on persuasion.

Examining narrativity at the feature level helps identify which aspects of stories are most effective. When using composite measures, both structural features (\textit{Agency} and \textit{Event Sequencing}) and response features (\textit{Suspense}, \textit{Curiosity}, and \textit{Surprise}) are positively related to persuasion. Structural features show a slightly stronger effect. Response features also contribute, but their effects are smaller on average.

The fine-grained analysis shows clear differences between individual narrative elements. \textit{Event Sequencing} and \textit{Curiosity} are the most positive predictors of persuasion when modeled as continuous features. This indicates that presenting events in a clear temporal order and creating engaging information gaps can particularly increase persuasion. \textit{Surprise} shows a mixed pattern: a higher \textit{Surprise} score is associated with lower persuasion, while the presence of \textit{Surprise} as a binary feature has a strong positive effect. This suggests that \textit{Surprise} can help persuasion when present, but may become less effective when overused. \textit{Agency} and \textit{Suspense} do not show strong independent effects once other narrative elements are taken into account.

Finally, the interaction analysis further clarifies how narrative features work together. Structural and response features show a significant negative interaction, meaning that they do not reinforce each other. When both feature types are already high, adding more of either yields smaller persuasive gains. This suggests that persuasion can be achieved through different narrative strategies, rather than by maximizing all narrative features at once.

In summary, the findings show that narrativity is a meaningful predictor of persuasion, with structure, reader engagement, and their interaction contributing in different ways.
